Text-image Alignment for Diffusion-based Perception

Diffusion models are generative models with impressive text-to-image synthesis capabilities and have spurred a new wave of creative methods for classical machine learning tasks. However, the best way to harness the perceptual knowledge of these generative models for visual tasks is still an open question. Specifically, it is unclear how to use the prompting interface when applying diffusion backbones to vision tasks. We find that automatically generated captions can improve text-image alignment and significantly enhance a model's cross-attention maps, leading to better perceptual performance. Our approach improves upon the current state-of-the-art (SOTA) in diffusion-based semantic segmentation on ADE20K and the current overall SOTA for depth estimation on NYUv2. Furthermore, our method generalizes to the cross-domain setting. We use model personalization and caption modifications to align our model to the target domain and find improvements over unaligned baselines. Our cross-domain object detection model, trained on Pascal VOC, achieves SOTA results on Watercolor2K. Our cross-domain segmentation method, trained on Cityscapes, achieves SOTA results on Dark Zurich-val and Nighttime Driving. Project page: https://www.vision.caltech.edu/tadp/. Code: https://github.com/damaggu/TADP.

==> tables/crossdomain_all.tex <==

% \begin{wraptable}[14]{r}{0.6\textwidth}
%   \vspace{-\baselineskip}
%   \centering
%   \small
%   \adjustbox{width=0.6\textwidth}{
%   \vspace{3pt}
%   \begin{tabular}{lcccccc}
%   \toprule
%     \multirow{2}{*}{Method} & Dark Zurich-val & ND & \multicolumn{2}{c}{Watercolor2k} & \multicolumn{2}{c}{Comic2k} \\
%     &  mIoU &  mIoU & mAP & AP$_{50}$ & mAP & AP$_{50}$ \\
%     \midrule
%     DAFormer \citep{hoyer_daformer_2022} & -- & 54.1 & -- & -- & -- & --\\
%     Refign-DAFormer \citep{bruggemann_refign_2022} & -- & 56.8 & -- & -- & -- & --\\
%     PTDiffSeg \citep{gong_prompting_2023} & 37.0 & -- & -- & -- & -- & --\\
%     FasterRCNN+CLIP \citep{vidit_clip_2023} & -- & -- & 43.4 & -- & 33.5 & -- \\
%     \midrule
% %    \textit{Ours} & & \\
%     \ours\textsubscript{null} & 40.8 & 57.6 & 56.3 & 87.8 & 45.2 & 78.0\\
%     \ours\textsubscript{simple} & 41.7 & 57.2 & 54.7 & 86.9 & 43.7 & 76.4\\
%     \ours\textsubscript{TextualInversion} & 41.7 & 58.1 & -- & -- & -- & --\\
%     \ours\textsubscript{DreamBooth} & \textbf{42.6} & \textbf{59.7} & \textbf{56.9} & \textbf{88.2} & \textbf{46.5} &  77.9\\
%     \midrule 
% %    \textit{Ablations} & & \\
%     \ours\textsubscript{NearbyDomain} & \textbf{42.6} & 57.9 & 52.4 & 86.3 & 45.0 & \textbf{78.4}\\
%     \ours\textsubscript{UnrelatedDomain} & 41.7 & 57.2 & 53.1 & 86.4 & 42.9 & 75.4\\
%     \bottomrule
%   \end{tabular}
%   }
%     \caption{\textbf{Cross-domain perception results.} We report the mIoU on Cityscapes to Dark Zurich and Nighttime Driving (ND). We report the mAP and AP@0.5 on Pascal VOC2012 to Watercolor2k and Comic2k.  Our method sets a new SOTA for all these tasks.}
%   \label{tab:cross-domain-all}
% \end{wraptable}

% \begin{table}[t]
%   \centering
%   \small
%     \caption{\textbf{Cross-domain perception results.} Cityscapes to Dark Zurich and Nighttime Driving (ND). We report the mIoU. Pascal VOC2012 to Watercolor2k and Comic2k. We report the AP and AP@0.5. Our method sets a new SOTA for DarkZurich, Nighttime Driving, and Watercolor2K.}
%     \label{tab:cross-domain-all}
%   \adjustbox{width=1.0\linewidth}{
%   \vspace{3pt}
%   \begin{tabular}{lcccccc}
%   \toprule
%     \multirow{2}{*}{Method} & Dark Zurich-val & ND & \multicolumn{2}{c}{Watercolor2k} & \multicolumn{2}{c}{Comic2k} \\
%     &  mIoU &  mIoU & AP & AP$_{50}$ & AP & AP$_{50}$ \\
%     \midrule
%     DAFormer \citep{hoyer_daformer_2022} & -- & 54.1 & -- & -- & -- & --\\
%     % (UDA-R) Refign-DAFormer \citep{bruggemann_refign_2022} & -- & 56.8 & -- & -- & -- & --\\
%     Refign-DAFormer \citep{bruggemann_refign_2022} & -- & 56.8 & -- & -- & -- & --\\
%     PTDiffSeg \citep{gong_prompting_2023} & 37.0 & -- & -- & -- & -- & --\\\midrule
%     % (SDG) FasterRCNN+CLIP \citep{vidit_clip_2023} & -- & -- & -- & 43.4 & -- & 33.5 \\

%     % (CDWSOD) H2FA R-CNN (extra) \citep{xu2022h2fa}  & -- & -- & -- & 62.2 & -- & 53.0 \\
%     (CDWSOD) PLGE \citep{ouyang2021pseudo}   & -- & -- & -- & 56.5 & -- & 41.7 \\
%     (CDWSOD) ICCM \citep{hou2021informative}   & -- & -- & -- & 57.4 & -- & 37.1 \\
%     (CDWSOD) H2FA R-CNN \citep{xu2022h2fa}  & -- & -- & -- & 59.9 & -- & 46.4 \\

%     (UDAOD) ADDA \citep{topal2022domain}  & -- & -- & -- & 49.8 & -- &  23.8 \\
%     (UDAOD) MCAR \citep{zhao2020adaptive}  & -- & -- & -- & 56.0 & -- & 33.5 \\
%     (UDAOD) UMT \citep{deng2021unbiased}  & -- & -- & -- & 58.1 & -- & -- \\
%     (UDAOD+extra Data) DASS-Detector \citep{topal2022domain}  & -- & -- & -- & 71.53 & -- & 64.25 \\

%     \midrule
% %    \textit{Ours} & & \\
%     \ours\textsubscript{null} & \textbf{42.8} & 57.5 & 42.1 & 72.1 & 31.1 & \textbf{57.4} \\
%     \ours\textsubscript{simple} & 39.1 & 56.9 & \textbf{43.5} & \textbf{72.2} & 31.9 & 56.6\\
%     \ours\textsubscript{TextualInversion} & 41.4 & \textbf{60.8} & 43.2 & \textbf{72.2} & \textbf{33.15} & \textbf{57.4}\\
%     \ours\textsubscript{DreamBooth} & 38.9 & 60.4 & 43.2 & \textbf{72.2} & 32.9 &  56.9\\
%     \midrule 
% %    \textit{Ablations} & & \\
%     \ours\textsubscript{NearbyDomain} & 41.9 & 56.9 & 42.0 & 71.5 & 31.8 & 56.4\\
%     \ours\textsubscript{UnrelatedDomain} & 42.33 & 55.1 & 42.2 & 71.9 & 32.0 & 55.9\\
%     \bottomrule
%   \end{tabular}
%   }

%   \vspace{-16pt}
% \end{table}

\begin{table}[t]
  \centering
  \small
  \caption{\textbf{Cross-domain perception results.} Cityscapes (CD) to Dark Zurich (DZ) val and Nighttime Driving (ND). We report the mIoU. Pascal VOC2012 to Watercolor2k and Comic2k. We report the AP and $AP_{50}$. Our method sets a new SOTA for DarkZurich, Nighttime Driving, and Watercolor2K.}
  \label{tab:cross-domain-all}
  \adjustbox{width=1.0\linewidth}{
  \vspace{3pt}
  \begin{tabular}{lcccccc}
  \toprule
    \multirow{2}{*}{Method} & Dark Zurich-val & ND & \multicolumn{2}{c}{Watercolor2k} & \multicolumn{2}{c}{Comic2k} \\
    &  mIoU &  mIoU & AP & AP$_{50}$ & AP & AP$_{50}$ \\
    \midrule
    DAFormer \citep{hoyer_daformer_2022} & -- & 54.1 & -- & -- & -- & --\\
    Refign-DAFormer \citep{bruggemann_refign_2022} & -- & 56.8 & -- & -- & -- & --\\
    PTDiffSeg \citep{gong_prompting_2023} & 37.0 & -- & -- & -- & -- & --\\
    \midrule
    \multicolumn{7}{l}{\textit{Cross domain weakly supervised object detection}}\\
    \midrule
    PLGE \citep{ouyang2021pseudo}   & -- & -- & -- & 56.5 & -- & 41.7 \\
    ICCM \citep{hou2021informative}   & -- & -- & -- & 57.4 & -- & 37.1 \\
    H2FA R-CNN \citep{xu2022h2fa}  & -- & -- & -- & 59.9 & -- & 46.4 \\
    \midrule
    \multicolumn{7}{l}{\textit{Unsupervised domain adaptation object detection}}\\
    \midrule
    ADDA \citep{topal2022domain}  & -- & -- & -- & 49.8 & -- &  23.8 \\
    MCAR \citep{zhao2020adaptive}  & -- & -- & -- & 56.0 & -- & 33.5 \\
    UMT \citep{deng2021unbiased}  & -- & -- & -- & 58.1 & -- & -- \\
    DASS-Detector (extra data) \citep{topal2022domain}  & -- & -- & -- & 71.5 & -- & \cellcolor{CBLightYellow}\textbf{64.2} \\
    \midrule
    \midrule
    \ours\textsubscript{null} & \textbf{42.8} & 57.5 & 42.1 & 72.1 & 31.1 & \textbf{57.4} \\
    \ours\textsubscript{simple} & 39.1 & 56.9 & \textbf{43.5} & \textbf{72.2} & 31.9 & 56.6\\
    \ours\textsubscript{TextualInversion} & 41.4 & \textbf{60.8} & 43.2 & \textbf{72.2} & \textbf{33.2} & \textbf{57.4}\\
    \ours\textsubscript{DreamBooth} & 38.9 & 60.4 & 43.2 & \textbf{72.2} & 32.9 &  56.9\\
    \midrule 
    \ours\textsubscript{NearbyDomain} & 41.9 & 56.9 & 42.0 & 71.5 & 31.8 & 56.4\\
    \ours\textsubscript{UnrelatedDomain} & 42.3 & 55.1 & 42.2 & 71.9 & 32.0 & 55.9\\
    \bottomrule
  \end{tabular}
  }
  \vspace{-16pt}
\end{table}


==> tables/results_subtable.tex <==
% \documentclass{article}
% \usepackage{subcaption}
% \usepackage{graphicx}


\begin{table}[h]
  % \centering
  \begin{subtable}{0.31\linewidth}
    \centering
    \adjustbox{max width=0.9\linewidth}{%
      \begin{tabular}{lcccccc}
      % Table content for subtable 1
      \toprule
      Method & Avg & TA & LS & G & OT & mIoU\textsuperscript{ss} \\
      \midrule
      VPD \citep{zhao_unleashing_2023} & \checkmark & \checkmark & & & \checkmark & 82.34 \\
      VPD(LS) & & & \checkmark & & \checkmark & 83.06 \\
      Class Embs & & & \checkmark &  & \checkmark & 82.72 \\
      Class Names & & & \checkmark & & \checkmark & 84.08 \\
      \ours-0  & & & \checkmark & \checkmark & & 86.36 \\
      \ours-20  & & & \checkmark & \checkmark & & 86.19 \\
      \ours-40  & & & \checkmark & \checkmark & & \textbf{87.11} \\
      \ours(NO)-20  & & & \checkmark & & & 86.35 \\
      \midrule
      \textit{\ours-Oracle} & & & \checkmark & & & 89.85 \\
      \bottomrule\\
      \end{tabular}
    }%
    \caption{\textbf{Prompting for Pascal VOC2012 Segmentation.} We report the single scale validation mIoU for Pascal experiments. Avg: EOS token averaging, TA: Text Adapter, LS: Latent Scaling, G: Grammar, OT: Off-target information. For our method, we indicate the minimum length of the BLIP caption with \ours-$X$ and nouns only with (NO).}
    \label{tab:pascal}%
  \end{subtable}%
  
  \hfill
  \begin{subtable}{0.31\textwidth}
    \centering
    \adjustbox{max width=0.9\linewidth}{%
    \begin{tabular}{lcccc}
    \toprule
%    \begin{tabu}to 1.1\linewidth{l*{5}{X[c]}}\toprule
    Method & \#Params & Crop & mIoU$^{\rm ss}$ & mIoU$^{\rm ms}$ \\
    \midrule
%    \addlinespace[3.0pt]
%    \multicolumn{5}{l}{\textit{supervised pre-training}}\\
%    Swin-L~\cite{liu_swin_2021}  &160K  & 640$^2$ & 647G & 52.1  & 53.5  \\
%    ConvNeXt-L~\cite{liu_convnet_2022} & 160K  & 640$^2$ & 614G & 53.2  & 53.7  \\
%    ConvNeXt-XL~\cite{liu_convnet_2022}  & 160K  &  640$^2$ & 834G & 53.6  & 54.0  \\  
%    \bottomrule
    \addlinespace[3.0pt]
    \multicolumn{5}{l}{\textit{self-supervised pre-training}}\\
    %\midrule
    %MAE-ViT-L/16~\cite{he_masked_2022} & -  &  - & 53.6  & - \\
    EVA \citep{fang_eva_2022} & 1.01B & 896$^2$ & 61.2 & 61.5 \\
    InternImage \citep{wang_internimage_2022} & 1.08B & 896$^2$ & \cellcolor{CBLightYellow}\textbf{62.5} & \textbf{62.9} \\ 
    \midrule
    \addlinespace[3.0pt]
    \multicolumn{5}{l}{\textit{multi-modal pre-training}}\\
    %\midrule
    CLIP-ViT-B \citep{rao_denseclip_2022} & 105M & 640$^2$ &  50.6 & 51.3 \\
    ViT-Adapter \citep{chen_vision_2022} & 571M & 896$^2$ & 61.2 & 61.5 \\
    BEiT-3 \citep{wang_image_2023} & 1.01B & 896$^2$ & \textbf{62.0} & 62.8 \\
    ONE-PEACE \citep{wang_one-peace_2023} & 1.52B & 896$^2$ & \textbf{62.0} & \cellcolor{CBLightYellow}\textbf{63.0} \\    
    \midrule
    \addlinespace[3.0pt]
    \multicolumn{5}{l}{\textit{diffusion-based pre-training}}\\
    %\midrule
    VPD$_{\rm A32}$ \citep{zhao_unleashing_2023}   & 862M & 512$^2$ & 53.7  & 54.6 \\
    VPD(R)   & 862M & 512$^2$ & 53.1  & 54.2 \\
    VPD(LS)   & 862M & 512$^2$ & 53.7  & 54.4 \\
    % Ours BLIP-0   & 80K & 512$^2$ & -- & 54.4  & 55.6 \\
    % Ours BLIP-20   & 80K & 512$^2$ & -- & 54.7  & 55.7 \\
    \rowcolor{CBLightGreen} \ours-40 (Ours) & 862M & 512$^2$ & \textbf{54.8}  &  \textbf{55.9} \\
    \midrule
    \textit{\ours-Oracle} & 862M & 512$^2$ & 72.0  & - \\
    \bottomrule
    %\end{tabu}
    \end{tabular}%
    }%
  \caption{\textbf{Semantic segmentation with different methods for ADE20k.} Our method (green) achieves SOTA within the diffusion-pretrained models category. The results of our oracle indicate the potential of diffusion-based models for future research as it is significantly higher than the overall SOTA (highlighted in yellow).}
  \label{tab:seg_ade_full}%
  \end{subtable}%
  \hfill
  
  \begin{subtable}{0.31\textwidth}
    \centering
    \adjustbox{max width=0.9\linewidth}{%
    \begin{tabular}{lcccccc}
    \toprule
    Method & RMSE$\downarrow$  & $\delta_1\uparrow$    & $\delta_2\uparrow$    & $\delta_3\uparrow$    & REL $\downarrow$  & log10 $\downarrow$ \\\midrule
    \multicolumn{7}{l}{\textit{default schedule}}\\
    \midrule
    SwinV2-L \citep{liu_swin_2021-1} & 0.287 & 0.949 & 0.994 & 0.999 & 0.083 & 0.035 \\
    AiT \citep{ning_all_2023} & 0.275 & 0.954 & 0.994 & 0.999 & 0.076 & 0.033\\
    ZoeDepth \citep{bhat_zoedepth_2023} & 0.270 & 0.955 & 0.995 & 0.999 & 0.075 & 0.032\\
    VPD \citep{zhao_unleashing_2023} & 0.254 & 0.964 & 0.995 & 0.999 & 0.069 & 0.030 \\
    \midrule
    VPD(R) & 0.248 & 0.965 & 0.995 & 0.999 & 0.068  & 0.029 \\
    VPD(LS) & 0.235 & 0.971 & 0.996 & 0.999 & 0.064  & 0.028 \\
    \rowcolor{CBLightGreen}\textbf{ours-40} & \textbf{0.225} & \textbf{0.976} & \textbf{0.997} & \textbf{0.999} & \textbf{0.062} & \textbf{0.027} \\
    \bottomrule
    \addlinespace[4.0pt]
    \multicolumn{7}{l}{\textit{fast schedule, 1 epoch}}\\
    \midrule
    VPD & 0.349 & 0.909 & 0.989 & 0.998 & 0.098 & 0.043 \\
    VPD(R) & 0.340 & 0.910 & 0.987 & 0.997 & 0.100 & 0.042\\
    VPD(LS) & 0.332 & 0.926 & 0.992 & 0.998 & 0.097 & 0.041 \\
    \rowcolor{CBLightGreen}\textbf{ours-0} & \textbf{0.328} & 0.935 & \textbf{0.993} & \textbf{0.999} & 0.082 & 0.038 \\
    \rowcolor{CBLightGreen}\textbf{ours(TA)-0} & 0.332 &\textbf{ 0.940} & 0.993 & \textbf{0.999} & \textbf{0.081}  & \textbf{0.036} \\
    \bottomrule
    \end{tabular}
    }%
    \caption{\textbf{Depth estimation in NYUv2.} We find that for depth estimation, latent scaling is particularly important, accounting for a relative gain of $\sim5.5\%$ on the RMSE metric. Improved image-text alignment also has a significant effect, improving $\sim4\%$ relative on the RMSE metric. We find that the longest BLIP captions we try, 40 tokens, perform the best. The same effects hold on the fast schedule, but are less pronounced.}
  \label{tab:depth}
  \end{subtable}
  % \caption{Three Subtables in a Row}
\end{table}

==> tables/seg_ade20k_fast.tex <==
\begin{table}[t]
  \centering
  %\vspace{3pt}
  \adjustbox{width=0.7\linewidth}{
    \begin{tabular}{lcccc}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{2}{c}{4K Iters} & \multicolumn{2}{c}{8K Iters} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}
          & mIoU$^{\rm ss}$ & mIoU$^{\rm ms}$ & mIoU$^{\rm ss}$ & mIoU$^{\rm ms}$ \\ \midrule
    VPD$_{\rm A32}$ \citep{zhao_unleashing_2023} & 43.1 & 44.2 & 48.7 & 49.5  \\
    VPD(R)          & 42.6 & 43.6 & 49.2 & 50.4 \\
    VPD(LS)        & 45.0 & 45.8 & 50.5 & 51.1 \\
    \rowcolor{CBLightGreen} \ours-20 (Ours)         & \textbf{50.2} & \textbf{50.9} & \textbf{52.8} & \textbf{54.1} \\
    \rowcolor{CBLightGreen}\ours(TA)-20 (Ours)    & 49.9 & 50.7 & 52.7 & 53.4 \\
    \bottomrule
    \end{tabular}
  }
\caption{\textbf{Semantic segmentation fast schedule.} Our method has a large advantage over prior work on the fast schedule with significantly better performance in both the single-scale and multi-scale evaluations for 4k and 8k iterations.}
\label{tab:seg_ade_fast}
  %\vspace{-10pt}
\end{table}
% \end{document}


==> tables/seg_ade_4k_ablations.tex <==
% Table skeleton generated by ChatGPT 
\definecolor{LightCyan}{rgb}{0.88,1,1}

\begin{table}
    \centering
    \small
    \adjustbox{width=0.4\linewidth}{
    \begin{tabular}{cc}
        & \textbf{Recall} \\
        \rotatebox[origin=c]{90}{\textbf{Precision}} &
        \begin{tabular}{c|c|c|c}
            & \textbf{0.50} & \textbf{0.75} & \textbf{1.00} \\
            \hline
            \rotatebox[origin=c]{90}{\textbf{  0.50  }} & 49.53 & 52.00 & 55.22 \\
            \hline
            \rotatebox[origin=c]{90}{\textbf{  0.75  }} & 49.17 & 51.46 & 58.62 \\
            \hline
            \rotatebox[origin=c]{90}{\textbf{  1.00  }} & 50.20 & 54.82 & \cellcolor{CBLightCyan} 63.29 \\
        \end{tabular} \\
    \end{tabular}
    }
      \caption{\textbf{ADE20K - Oracle Precision-Recall Ablations} We modify the oracle captions by randomly adding or removing classes such that the precision and recall is 0.50, 0.75 or 1.00. We train models on ADE20K on the fast schedule (4K) using these captions. The 4k iteration oracle equivalent is highlighted in blue.}
    \label{tab:oracle_ablations}
\end{table}
